Leaky Cauldron on the Dark Land: Understanding Memory Side-Channel Hazards in SGX

Side-channel risks of Intel's SGX have recently attracted great attention. Under the spotlight is the newly discovered page-fault attack, in which an OS-level adversary induces page faults to observe the page-level access patterns of a protected process running in an SGX enclave. With almost all proposed defense focusing on this attack, little is known about whether such efforts indeed raise the bar for the adversary, whether a simple variation of the attack renders all protection ineffective, not to mention an in-depth understanding of other attack surfaces in the SGX system. In the paper, we report the first step toward systematic analyses of side-channel threats that SGX faces, focusing on the risks associated with its memory management. Our research identifies 8 potential attack vectors, ranging from TLB to DRAM modules. More importantly, we highlight the common misunderstandings about SGX memory side channels, demonstrating that high frequent AEXs can be avoided when recovering EdDSA secret key through a new page channel and fine-grained monitoring of enclave programs (at the level of 64B) can be done through combining both cache and cross-enclave DRAM channels. Our findings reveal the gap between the ongoing security research on SGX and its side-channel weaknesses, redefine the side-channel threat model for secure enclaves, and can provoke a discussion on when to use such a system and how to use it securely.

==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.


==> tex/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	ccs-template.tex 

PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf}

all:  ${PDF}

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do 	pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'


==> tex/attack3.tex <==
\subsection{Leaky Address Translation}
\label{subsec:tlb}

Our study on Vector~\ref{vector:tlb1} reveals a TLB probing attack against SGX
enclaves, which has \textit{never been implemented before}.  The attack succeeds
when HyperThreading is turned on, launched from one logical core to another on the same
physical core. On the future systems where PCID-based flushing is enabled
(Vector \ref{vector:tlb2}), such attacks can also be conducted without
HyperThreading.

\vspace{3pt}\noindent\textbf{Attack techniques}.
We developed a \textit{novel} technique that allows us to probe the iTLB and
dTLB at the same time. Specifically, on our testbed, bits 12$\sim$15 of a
virtual address on a data page determine the dTLB set; bits 12$\sim$14 of a
virtual address on a code page determine the iTLB set. Instead of using
\texttt{rdtsc} based time measurements, we used performance counters to monitor
dTLB and iTLB misses.  To simplify our description, we define a TLB eviction set
as a set of pages whose address translation data will be mapped to the same TLB
set. We built 8 iTLB eviction sets and 16 dTLB eviction sets by allocating 128
contiguous virtual pages. We developed the code to probe iTLB and dTLB at the
same time, compiled the code into binary, and then copied the binary code on to
one of iTLB eviction sets (the control flow will jump from one page to the next
in the same eviction set). The other iTLB eviction sets were processed similarly.
Finally, we made the iTLB-eviction-set pages as executable pages. As such, when
the code ran within one iTLB eviction set, it first checks performance counters
to detect the existing value of iTLB and dTLB misses, and then probes the
current iTLB set by executing itself. At the same time, it probes one of the
dTLB sets. In executing the last page of this iTLB eviction set, the performance
counters will be read again to determine the iTLB misses and dTLB misses, and the
results of the dTLB and iTLB misses are recorded to the corresponding dTLB
%counters will be read again to determine the iTLB and dTLB misses, and the results of the iTLB and dTLB misses are recorded to the corresponding dTLB
eviction set so that dTLB pollution is avoided.  The control flow then jumps to
probing the next iTLB eviction set. As there are more dTLB sets than the iTLB
sets, the code probes all 16 dTLB eviction sets in two iterations of iTLB
probing.


%\vspace{3pt}\noindent\textbf{Attack techniques}.
%On our testbed, bits 12$\sim$15 of a virtual address on a data page determine
%the dTLB set; bits 12$\sim$14 on a virtual address of a code page determine the
%iTLB set. We used performance counters to monitor dTLB and iTLB misses. We built
%our TLB eviction set as follows: first we allocated 64 contiguous virtual pages
%for iTLB eviction set; then we copied the binary code for probing the dTLB onto
%these pages; then we set these pages as executable pages. As such, when the code
%ran within one instruction page, it also \primeprobe one dTLB set, and recorded
%the number of dTLB misses. The last code page would jumped back to the first
%page. We arranged the eviction pages to \primeprobe all 8 iTLB sets and 16 dTLB
%sets in a single iteration.

%We recorded the performance counter to data pages which we used as dTLB eviction set to avoid dTLB pollution. If  the victim enclave located in another logical core accessed pages in a TLB set, it would evict TLB entries in our logical core,  consequently we would observe an increase of TLB misses while probing the TLB set.

\ignore{To build such an attack,
\yinqian{@Guoxing, how did you do the attack?} we set performance
counters to monitor dTLB and iTLB misses.  The TLB \primeprobe code is distributed in $64$
contiguous pages that are grouped into $8$ sets. Each set contains $8$ pages
sharing the same iTLB set. The attack code will first move from one page to the next
within the same set. When the last page of a set is reached, it will jump to
the first page of the next set. When the execution hits the last page of the last set, the code
will jump to the first page of the first set until a predefined iteration number
is met. While the code runs within one set, it will also access $4$ data pages
that share the same dTLB set, and record performance counter reads.
Specifically, on the first code page in one set, performance counter reads are
recorded. $4$ data pages are accessed within next several code pages. In the
last code page of that set, performance counter reads are recorded again before the attack code
jump to next set. Note that performance counter reads were written to the same
data pages we accessed to avoid dTLB pollution. A performance counter read
increase will be observed if the victim that located in another logical core of
the same physical core accesses one page that shares the same TLB set with the
pages we accessed.}


\vspace{5pt}\noindent\textbf{Examples}. To demonstrate the attack, we
implemented a simple binary search algorithm inside an enclave. Specifically,
16384 integers were sorted and stored in 16 contiguous virtual pages.  Reading
the integers leads to address translation using TLBs.  In our experiment we
monitored every one of the 16 dTLB sets every 7000 CPU cycles. Although the page
access pattern does not leak enough information for us to determine which
integer was searched, based upon the traces we observed, we were able to
partition all 16384 numbers into 9 categories and reliably determine which
category the searched one belongs to.
%partition the 16384 integers into 9 categories and reliably determine which category the searched integer belongs to.



%\vspace{5pt}\noindent\textbf{Examples}. To demonstrate the attack, we implemented a simple binary search algorithm inside an enclave. Specifically, 16384($=2^{14}$) integers were sorted and stored in 16 contiguous virtual pages. Reading the integers located would result in accessing pages whose address translation information is stored in the TLB.  In our experiment we monitored every one of the 16 dTLB sets every 7000 CPU cycles. Although the page access pattern does not leak enough information for us to determine which integer was searched, however, according to the traces we observed, we were able to partition the 16384 integers into 9 categories and reliably determine which category the searched integer belongs to. This example demonstrates that information leakage is possible through TLB probing attacks.

%As an example, we implement a covert channel. We write an enclave code that
%repeatedly access two data pages with address [base\_addr] and [base\_addr +
%0x1000 * i], $i = 0, \dots, 7$ to communicate the number $i$ to our TLB
%\texttt{Prime+Probe} code. The attack code observes dTLB misses for two dTLB
%sets and $i$ can be successfully recovered by calculating the difference
%between the dTLB set indexes.




















%---------------------------------------------------------------------------------------------------



\ignore{

In this section, we describe TLB probing attacks against SGX enclaves. Our
demonstrated attacks are performed with HyperThreading enabled, from one logical
core to another logical core. On machines where Attack Vector \ref{vector:tlb2}
is enabled, such attacks can also be conducted without HyperThreading.
Unfortunately we do not have such computers to test the attacks.

\vspace{5pt}\noindent\textbf{Attack techniques}.
To the best of our knowledge, there is no described or demonstrated
TLB probing attacks. Therefore, our construction of TLB probing attacks
Specially, \yinqian{@Guoxing, how did you do the attack?} We set performance
counters to monitor DTLB and ITLB misses. On our testbed bits 12$\sim$15 of a
virtual address determine a DTLB set; bits 12$\sim$14 of a virtual address
determine a ITLB set. The TLB \texttt{Prime+Probe} Code is distributed in $64$
contiguous pages that are grouped into $8$ sets. Each set contains $8$ pages
sharing the same ITLB set. Code will first jump from one page to the next page
within the same set. When code reaches the last page of one set, it will jump to
the first page of next set. When code reaches the last page of the last set, it
will jump to the first page of the first set until a predefined iteration number
is met. While the code runs within one set, it will also access $4$ data pages
that share the same DTLB set, and record performance counter reads.
Specifically, in the first code page of one set, performance counter reads are
recorded. $4$ data pages are accessed within next several code pages. In the
last code page of that set, performance counter reads are recorded again before
jump to next set. Note that performance counter reads are written to the same
data pages we accessed to avoid DTLB pollution. A performance counter read
increase will be observed if a victim that located in another logical core of
the same physical core access one page that share the same TLB set with the
pages we accessed.


\vspace{5pt}\noindent\textbf{Examples}.
\yinqian{@Guoxing, what examples are demonstrated?}
As an example, we implement a covert channel. We write an enclave code that repeatedly access two data pages with address [base\_addr] and [base\_addr + 0x1000 * i], $i = 0, \dots, 7$ to communicate the number $i$ to our TLB \texttt{Prime+Probe} code. In our TLB \texttt{Prime+Probe} code, DTLB misses are observed for two DTLB sets and $i$  can be successfully recovered by calculating the difference between the DTLB set indexes.}


==> tex/comparison.tex <==
\section{Comparison with existing work on side (controlled) channel attacks on SGX}

==> tex/evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}



==> tex/measure.tex <==
\section{Understanding and Defense Insights}
\label{sec:measure}

\subsection{Understanding the Threats}
\label{subsec:understand}

\vspace{5pt}\noindent\textbf{Application and library collection}.

\vspace{5pt}\noindent\textbf{Methodology}. 


\vspace{5pt}\noindent\textbf{Findings}.



\subsection{Mitigation Options}
\label{subsec:defense}


\vspace{5pt}\noindent\textbf{Challenges and potential solutions}. 



\vspace{5pt}\noindent\textbf{Example: in-enclave detection}. 
